The Links Have It: Infobox Generation by Summarization over Linked Entities

Online encyclopedia such as Wikipedia has become one of the best sources of knowledge. Much effort has been devoted to expanding and enriching the structured data by automatic information extraction from unstructured text in Wikipedia. Although remarkable progresses have been made, their effectiveness and efficiency is still limited as they try to tackle an extremely difficult natural language understanding problems and heavily relies on supervised learning approaches which require large amount effort to label the training data. In this paper, instead of performing information extraction over unstructured natural language text directly, we focus on a rich set of semi-structured data in Wikipedia articles: linked entities. The idea of this paper is the following: If we can summarize the relationship between the entity and its linked entities, we immediately harvest some of the most important information about the entity. To this end, we propose a novel rank aggregation approach to remove noise, an effective clustering and labeling algorithm to extract knowledge.

==> section5.tex <==
% !TEX root = entity_clustering.tex

\section{Scalability}
The clustering procedure needs to be conducted on each entity. The straightforward approach executes the clustering procedure for each entity {\it repeatedly} and {\it independently}. In general, the clustering procedure needs to be executed millions of time, which may incur unaffordable huge time. In this section, we first show that linked entities usually have significant overlaps in their neighbors, which allows us to reuse the clustering result generated earlier if an appropriate order is posed on the clustering tasks.  We propose a best linear order model to find the best order so that we can boost the execution of millions clustering tasks.

\paragraph*{Problem Statement}
Given set of articles $S$ and cluster-then-label method, we want to produce knowledge from $S$ efficiently, which outputs clusters and labels for all articles in $S$. To handle scalability, we use MST(maximal spanning tree) based cluster reuse strategy, which stores some clusters and can be reused by its overlapped entities.

\subsection{Motivations}
We first present our observation that {\it clusters of linked entities usually overlap with each other.} Thus, if we can define a good order to cluster for entities, we may reuse the previously produced clustering result. We first show that linked entities in a real knowledge base tend to share a significant number of neighbors. We calculate the maximal neighbor overlap for each article, which is the maximal overlap among all its linked entities. The overlap between an entity pair is calculated by Eq.~\ref{eq:overlap}. In Figure~\ref{fig:hop_a} we show the cumulative distribution of the maximal neighbor overlap, where point in the the curve stands for percentage of articles whose maximal neighbor overlap less than the value on x-axis. We find that nearly 70\% articles whose maximal neighbor overlap is larger than 0, and 15\% whose maximal neighbor overlap is 1. %{\bf We also give the cumulative distribution of a randomized network preserving the degree sequence of the Wiki knowledge graph. Compared to the null model, the observed overlap in the real knowledge graph is statistically significant enough.}

\begin{figure} \centering
\subfigure[\small{Maximal neighbor overlap.}] { \label{fig:hop_a}
\includegraphics[width=0.45\columnwidth,height=0.3\columnwidth]{maximalNeighborOverlap.eps}
}
\subfigure[\small{Overlap for k-hop neighbor.}] { \label{fig:hop_b}
\includegraphics[width=0.45\columnwidth,height=0.3\columnwidth]{khopoverlap.eps}
}
\caption{Overlap Distribution. }
\label{fig:entity_overlap}
\end{figure}

The above observation implies a better strategy: {\it reusing previous clustering results}. That is when a set of linked entities of an entity need to be clustered, we first scan the previous clusters that can be reused before direct clustering. Obviously, this approach can save a lot of computation cost if significant overlapping exists.

One naive implementation of above reusing strategy is memorizing all the previously generated clustering results. Anytime when a new entity $c$ comes and its neighbors $N(c)$ needs to be clustered, we first find $c'$ who shares the most neighbors with $c$ from the previous proceeded entities. The clustering results of the overlapping part will be directly inherited and we only need cluster the remaining part.
Finally, a sort of combination procedure needs to be executed to generate the final clustering for $N(c)$. However, this naive approach has two weaknesses.
\begin{itemize}
\item First, {\it it is costly}. It needs $O(E)$ space to memorize the previous results, which in turn incurs $O(N^2)$ time to fetch the most overlapped entities even ignoring the time to calculate the overlap.
\item Second, {\it memorizing all previous clustering results is unnecessary}. Actually, a random pair of entity in general shares tiny overlap. We show in Figure~\ref{fig:hop_b} the average overlap ratio between an entity and its $k$-hop neighbors. We use entity $Steve\ Jobs,\ Apple\ Inc.,\ Shanghai$ as examples. Their average overlap ratios are $0.088,\ 0.062,\ 0.042$, respectively. When $k$ increases, the overlap fast converges to zero. Thus, an arbitrary entity pair is of low probability to share many neighbors, which make the memorization of all previous clusters unnecessary.
\end{itemize}


To overcome the above weaknesses, we propose to find a best linear order to process each entities and only memorize the immediately prior clustering result. Memorizing one result improves the performance. The best linear order ensures the effectiveness of the reuse.

\subsection{Problem Models}
To define the best linear order, we first need to define a measurement of the confidence that a pair of entities should be clustered consecutively. Clearly, the overlap ratio between the neighbors is a direct indicator. The more common neighbor two entities share, the more clustering result can be reused. Since only linked entity pairs are possible to have significant overlap, we only define the neighborhood overlap ratio on two entities $u, v$ such that $u$ has a link to $v$ in Wiki by the following Jaccard index:
\begin{equation}
\label{eq:overlap}
J(u\rightarrow v)=\frac{|N(u)\cap N(v)|}{|N(v)|}
\end{equation}
, where $N(u)$ is the neighbors of $u$ in the knowledge graph. We highlight that the Jaccard is not symmetric since we use $|N(v)|$ as the denominator. The above Jaccard index characterizes how much $v$ can inherit $u$'s result. The closer $N(u)\cap N(v)$
to $N(v)$, the more deserved that $v$ inherits $u$'s result.

\paragraph*{Entity Correlated Graph}
Based on the above measure, we defined an entity correlated graph to encode the overlapping information for all linked entity pairs. Given these concepts, we propose {\it best inheritance order} problem to find a best linear order to cluster all entities.

\begin{definition}[$\tau$ Entity correlated graph ($\tau$-ECG)]
A $\tau$-ECG is an edge weighted graph $G(V, E, w)$, where $V$ represents set of entities, $E$ represents the set of direct hyperlinked such that $w(u\rightarrow v)>\tau$, where $w(u, v)=J(u, v)$ and $\tau$ is a parameter.
\end{definition}

To construct $\tau$-ECG, we just need to scan each directed edge of the knowledge graph. For each direct edge $u\rightarrow v$, $O(|N(u)|+|N(v)|)$ time cost is necessary to calculate the Jaccard index. Since in real knowledge graphs, the maximal degree is usually bounded. Such cost can be considered as a constant. Thus, overall $O(|E|)$ cost is necessary to construct the graph.

% Actually, we can learn from figure~\ref{fig:hop_b} that overlap between entity pair decrease as the steps of neighbor increase. Take $Shanghai$ for example, average overlap for 1-hop neighbors is $0.088$, and $0.029$ for 2-hop neighbors, and close to $0$ on 10-hop neighbors. So taking 1-hop neighbors into consideration is reasonable. Here we reduce the computing complexity from $O(N^2)$ to $O(kN)$ or $O(|E|)$ where $k$ is constant, represents average number of linked entities.

In the definition of $\tau$-ECG, we use $\tau$ to tune the size of the resulting ECG.
A larger $\tau$ generally leads to a smaller ECG. We can also further reduce the construction cost of ECG by $\tau$. Specifically, with $\tau$ Jaccard computation can be reduced from $O(|N(u)|+|N(v)|)$ to $O(1)$ by the following upper bound estimation:
\begin{equation}
\label{eq:upp}
\frac{|N(u)\cap N(v)|}{|N(v)|} \leq \frac{\min\{|N(v)|,|N(u)|\}}{|N(v)|}
\end{equation} We can filter some entity pairs by just the degree of two entities. For example, if $\tau=0.1$ and degree for source and target entity is 10 and 100, respectively, then their Jaccard will not be larger than 0.1, thus  can be pruned.


We set the bound $\tau=0.05$ to construct the $ECG$. Because our experiment result (Figure.~\ref{fig:time_degree}) show that the reuse strategy may use more time than non-reuse strategy if the overlap is smaller than 0.05.



% we consider the cluster propagation, the base of cluster propagation is the common entities, and the more common entities, the obvious cluster propagation performs than direct clustering. So if the common entities are too small, hence small overlap, propagate clusters on these paths are insignificant. We can define $\tau-ECG$, where $\tau$ is the lower bound for generating edge.

\paragraph*{Model}
Now we are ready to formalize the problem model to find the best linear order to execute the clustering tasks. We refer to the problem as {\it best inheritance order } (BIO):
\begin{definition}[Best Inheritance Order (BIO)]
Given a $\tau-$ECG $G(V,E,w)$, find a linear order  $\zeta$ on $V$, such that\\
$\sum_{i=1}^N w(\zeta^{-1}(i),\zeta^{-1}(i+1) )$ is maximized.
\end{definition}

Clearly, BIO is equivalent to the {\it maximal hamilton path} (MHP) problem, which is a well-known NP-hard problem. To avoid the NP-Completeness of BIO, we propose an alternative problem model (BIT), which can be solved efficiently without sacrificing the effectiveness of the result.

The basic idea of BIT is that finding a partial order on nodes of ECG instead of a linear order. A partial order is equivalent to a rooted tree. Any path starting from the root encodes the information of the partial order. Given the tree, we ensure that each node can only inherits the clustering results of its parent.
%The rationality of the partial order comes from the observation that there is no obvious superiority of one node to another when the clustering task of some other node has been executed.For example, {\bf give an example}

\begin{definition}[Best Inheritance Tree (BIT)]
Given a $\tau$-ECG $G(V,E,w)$, find a spanning tree $T(V, E_T)$ of $G$ such that $\sum_{i=1}^{|E^{'}|} w(E_i^{'})$ is maximized.
\end{definition}

Clearly, BIT is the maximal spanning tree (MST) problem, whose optimal solution can be found in polynomial time. It was shown that for the same ECG, the optimal solution of BIT is prior to the optimal solution of BIO, which is stated in Lemma~\ref{lem:prio}. It is obvious because BIO is equivalent to traveling salesman problem, whose lower bound is minimal spanning tree~\cite{appro_mst}.

\begin{lemma}Given an ECG $G$, the optimal solution of $BIO(G)$
$$opt_{BIO}(G)\leq opt_{BIT}(G)$$, where $opt_{BIO}(G)$ and $opt_{BIT}(G)$ are the maximal weight of the optimal solution to $BIO(G)$ and $BIT(G)$, respectively.
\label{lem:prio}
\end{lemma}


\subsection{Solutions}
In this subsection, we first elaborate the MST based solution to solve BIT.
Given the partial order generated in the above step, we need to execute the clustering tasks on entities.  We also need a procedure to implement the inheritance of the clustering result from a node to its children, which will be elaborate in the second part of this section.

\subsubsection{MST based approach}
We give the basic idea to solve BIT. Given an ECG graph $G(V,E)$, we first use Prim algorithm to generate a maximal spanning tree $T(V,E^{'})$. We distinguish the first node selected in the Prim algorithm as the root node of $T$.
Given the MST tree $T$, we execute the clustering tasks level by level. Each node inherits the clustering result of its parent.  Each level memorizes the clustering result of each node in its parent level. When clustering for nodes in the $h$-th level, all the clustering results of the current level is memorized and can only be freed when $(h+1)$-th level is finished.

The Prim algorithm works as follows. Prim algorithm keeps a visited node set $S$. The algorithm first select a node as the root and add it into $S$. Then, the algorithm iteratively select an unvisited node in $V$ that owns a maximal edge weight to any nodes in $S$, and add it into $S$. The iteration terminates when all nodes in $V$ are visited. Note that this model will get a forest finally, and each forest may represent a semantic group. Because model is carried out on $\tau-ECG$, weak link between entity pair will be blocked by noisy link filtering and minimal overlap bound $\tau$.

We select the node with highest degree as the root of the MST tree. The rationality of this strategy is that a node with more neighbors can be more influential and its clusters can be inherited by more nodes.

We give an example in Figure~\ref{fig:bit_gen}. The graph consists of 6 nodes $a, b, c, d, e, f$, and each edge weight represents the overlap ratio between the two ending nodes. We first select node $b$ as the root since it is one of the nodes with the largest degree. Then we add $a, c, d, f, e$ in turn into the tree. In this way, we get the maximal spanning tree as shown in Figure~\ref{fig:bit_b}. Given the MST, we can propagate the clusters according to the tree path. We first cluster the linked entities of node $b$, then propagate the cluster results to nodes $a, c, d$, and node $d$ propagate the cluster results to node $e, f$.
\begin{figure} \centering
\subfigure[\small{Entity correlated graph.}] { \label{fig:bit_a}
\includegraphics[width=0.45\columnwidth]{ecg.eps}
}
\subfigure[\small{Best Inheritance Tree.}] { \label{fig:bit_b}
\includegraphics[width=0.45\columnwidth]{mst.eps}
}
\caption{Generate BIT from ECG.}
\label{fig:bit_gen}
\end{figure}

The space cost necessary for the memorization of previously generated clustering results is $O(w(T)\zeta(G))$, where $w(T)$ is the width of $T$ (the maximal level width of the tree) and the $\zeta(G)$ is the maximal degree of $G$. Clearly, $w(T)$ is upper bounded by $\zeta(G)$. Hence, we have the space cost of the MST approach is $O(\zeta(G)^2)$. In most real knowledge graphs, $\zeta(G)$ can be considered as a constant. Hence such space cost is acceptable in reality.

\subsubsection{Inheritance procedure}
Now we elaborate how to reuse cluster results on given a MST generated above.
Suppose a node $u$ needs to inherit the clustering result of its parent node $v$. Let $C(v)$ be the clustering result of $v$.  We next elaborate how $u$ inherits $v$'s result. The procedure is given in the inner loop of the algorithm. The inheritance procedure has three major steps. In the first step, it directly inherits the clustering result of the parent node. Specifically, for each $e\in N(u)\cap N(v)$, $e$ is assigned to the cluster of $v$ that contains $e$ and assigned with the corresponding cluster label. Let the clustering result of this step be $R_1=\{<C_i, l_i>\}$.  In the second step, for entities in $N(v)-N(u)$, we use our clustering-then-labeling approach generate its corresponding clusters and labels. Let the result be $R_2=\{<C'_i, l'_i>\}$. In the third step, we merge $R_1$ with $R_2$. In this step, we merge any two clusters from $C_i$ and $C'_j$ that share the same label. Let the result of this step be $R_1\cup R_2$. We finally return $R_1\cup R_2$ as the clustering result of $v$.

\paragraph*{Time Complexity}
Then we analysis the complexity of this procedure compared to direct clustering. The time complexity of Gmeans is $O(2KNID)$, where $K$ is the number of clusters, $N$ is the number of datapoints, $I$ is the number of iterations and $D$ is the dimension of attributes. For above procedure, suppose number of linked entities for $v$ and $u$ is $N_v$ and $N_u$, number of clusters for $v$ and $u$ is $K_v$ and $K_u$. Then for node $u$ time cost on direct clustering is $O(2K_uN_uID)$, and memory cost is 0. Time cost on inheritance procedure is $O(N_u\dot K_v)+O(2K_u^1N_u^1ID)$, where $N_u^1$ is number of nodes not being inherited from $v$ and $K_u^1$ is the number of clusters gen from these nodes. Time cost for inheritance procedure is $O(N_v)$ since we need memory all nodes in each clusters.

Note that time complexity of this procedure mainly rely on $N_u^1$. If $N_u^1=0$, which means all nodes can inherit from $v$, then total complexity is $O(N_u\dot K_v)$. But if $N_u^1=N_u$, which means no nodes can inherit from $v$, then total complexity is $O(N_u\dot K_v)+O(2K_uN_uID)$. 
